Towards Ranking Schemas by Focus

The main goal of this paper is to evaluate knowledge base schemas, modeled as a set of entity types, each such type being associated with a set of properties, according to their focus. We intuitively model the notion of focus as ''the state or quality of being relevant in storing and retrieving information''. This definition of focus is adapted from the notion of ''categorization purpose'', as first defined in cognitive psychology, thus giving us a high level of understandability on the side of users. In turn, this notion is formalized based on a set of knowledge metrics that, for any given focus, rank knowledge base schemas according to their quality. We apply the proposed methodology to more than 200 state-of-the-art knowledge base schemas. The experimental results show the utility of our approach

==> abstract-draft.tex <==
It is proven that knowledge representation schemas are essential formalisms in the representation of the internal conceptual components of a knowledge base. One of the main purposes of these data structures is to categorize information about real world objects. This is the very same purpose of what psychologist call ``categorization'', namely a means of organizing our mental life, of reducing the load on memory, and of helping us to store and retrieve information efficiently. In  this  paper, taking inspiration from the work in cognitive psychology, we define the ``categorization purpose'' as \textit{focus} and, in order to to  support an accurate level of schema reuse, we propose a solution to rank schemas according to their focus. Three are the main contributions: i) a cognitive psychology grounded account of the notion of focus; ii) a definition of focus in terms of three main computational tasks; iii) a prototype of a schema ranking system that applies a set of metrics to rate each schema according to their focus; iv) an evaluation  of the  application  of  the  ranking  system over  a  huge  amount  of  state-of-the-art  datasets.

introduce the notion of focus as 

in  order  to  support an accurate level of schema reuse we introduce the notion of focus as ``categorization'' 

propose a prototype of a schema ranking system that applies 


a set of metrics to rate each schema according to their categorization “relevance”. The main contributions are:

communicate and share meaning. 


Due to the difficulty and cost of designing these useful data structures, facilitating their reuse is becoming a pivotal challenge.

So far, in order to minimise the effort in building schemas, a huge number of solutions to facilitate their reuse [Ref.] have been provided. 

The facilities provided by these solutions are very valuable especially in the contextof theirstructural evaluation[Ref.].

KR schemas provide high-performance solutions to large scale categorization problems, namely problems of efficient information storage and retrieval. 

According to psychologist, \textit{categorization is the means by which we organize our mental life}. Communication and meaning heavily depend on it

the purpose of \textit{categorization} is at the basis of the organization of our mental life: meaning and communication heavily depend on it. In the context of AI this purpose of categorization is usually implemented by well defined and effective information objects, namely knowledge representation (KR) schemas. Due to the difficulty and cost of designing these useful data structures, facilitating their reuse is becoming a pivotal challenge.

In this paper we present a (quantitative) approach to evaluate and rank schemas analysing one of their most claimed purposes, namely their \textit{purpose of categorizing information about real world objects}. This purpose being what is necessary for putting information about things into categories and being what makes schemas valuable mechanisms for managing and searching information.

high-performance solutions to large scale categorization problems, namely problems of efficient information storageand retrieval. 
000


It is proven that knowledge representation schemas are essential formalisms in the representation of the internal conceptual components of a knowledge base. This data structures are very useful for enabling the management of the information inside the knowledge base and the searching of these information, even across multiple applications. So far, a huge, ever-growing, number of heterogeneous schemas has been produced. Due to the difficulty and cost of designing these useful data structures, facilitating their reuse is becoming a pivotal challenge and a lot of methods, search engines and catalogs have been created to address this issue. In this paper we present a (quantitative) approach to evaluate and rank schemas analysing one of their most claimed purposes, namely their \textit{purpose of categorizing information about real world objects}. This purpose being what is necessary for putting information about things into categories and being what makes schemas valuable mechanisms for managing and searching information.

==> abstract-ok.tex <==
\begin{abstract}
It is proven that \textit{knowledge representation schemas} are
high-performance solutions to large scale categorization problems, namely problems of efficient information storage and retrieval.
The main goal of this paper is to evaluate knowledge representation schemas according to their categorization purpose, in order to support an accurate level of their classification and reuse. To achieve this goal we take inspiration from the work in cognitive psychology and we define the schema ``categorization relevance'' as \textit{focus}. We then propose a solution to rank schemas according to their focus that is articulated into three main contributions: \textit{i)} a cognitive psychology grounded account of the notion of focus; \textit{ii)} a prototype of a schema ranking method that applies a set of metrics to rate each schema according to its focus; \textit{iii)} an analysis of the application of the ranking system over a huge amount of state-of-the-art data sets. Finally, through empirical results we show the utility of the proposed ranking method on three main tasks, namely \textit{Schema Ranking}, \textit{Schema Tagging} and \textit{Entity Type Recognition.} 
\end{abstract}


It is proven that \textit{knowledge representation schemas} are
high-performance solutions to large scale categorization problems, namely problems of efficient information storage and retrieval.
The main goal of this paper is to evaluate knowledge representation schemas according to their categorization purpose, in order to to support an accurate level of their reuse and decrease the effort on schemas construction. To achieve this goal we take inspiration from the work in cognitive psychology, we define the schema, ``categorization purpose'' as \textit{focus}, and we then propose a solution to rank schemas according to their focus. Three are the main contributions: \textit{i)} a cognitive psychology grounded account of the notion of focus; \textit{ii)} a definition of focus in terms of three main computational tasks; \textit{iii)} a prototype of a schema ranking system that applies a set of metrics to rate each schema according to their focus; \textit{iv)} an evaluation of the application of the ranking system over a huge amount of state-of-the-art data sets.

The main goal of this paper is to evaluate the relevance of knowledge representation schemas in addressing categorization problems,


in order to support an accurate level of their reuse and decrease the effort on schemas construction. 




It is proven that \textit{knowledge representation schemas} are essential formalisms in the representation of the internal conceptual components of a knowledge base. One of the main purposes of these data structures is to categorize information about real world objects. This is the very same purpose of what psychologists call \textit{``categorization''}, namely a \textit{``means of organizing our mental life and of helping us to store and retrieve information efficiently''}. 

The main goal of this paper is to evaluate knowledge representation schemas according to their categorization purpose, in order to to support an accurate level of their reuse and decrease the effort on schemas construction. To achieve this goal we take inspiration from the work in cognitive psychology, we define the schema, ``categorization purpose'' as \textit{focus}, and we then propose a solution to rank schemas according to their focus. Three are the main contributions: \textit{i)} a cognitive psychology grounded account of the notion of focus; \textit{ii)} a definition of focus in terms of three main computational tasks; \textit{iii)} a prototype of a schema ranking system that applies a set of metrics to rate each schema according to their focus; \textit{iv)} an evaluation of the application of the ranking system over a huge amount of state-of-the-art data sets.

==> misc/metrics.tex <==
Given the definitions of \textit{Cues} for entity types, we capture \textit{the categorization relevance of an entity type}, with the notion of $Focus(e)$, which we define as follows: 

\vspace{-0.2cm}
\begin{equation}
\small
Focus(e) = Cue_{e}^{'}(e) + Cue_{er}^{'}(e)
\vspace{-0.05cm}
\end{equation}

where $Cue_{e}^{'}(e)$ is a \textit{mean normalization} of $Cue_{e}(e)$, considering all the $Cue_{e}(e)$ values from a given set of KBSs $\left \{ K \right \}$, namely:

\vspace{-0.2cm}
\begin{equation}
\small
Cue_{e}^{'}(e) =\frac{Cue_{e}(e) - Cue_{e}(e_{i})_{average}}{Cue_{e}(e_{j})_{max} - Cue_{e}(e_{k})_{min}}
\vspace{-0.05cm}
\end{equation}

and where $Cue_{er}^{'}(e)$ is a \textit{min-max normalization} of $Cue_{er}(e)$ considering all the $Cue_{er}(e)$ values from a given set of KBSs $\left \{ K \right \}$, namely:

\vspace{-0.2cm}
\begin{equation}
\small
Cue_{er}^{'}(e) =\frac{Cue_{er}(e) - Cue_{er}(e_{i})_{min}}{Cue_{er}(e_{j})_{max} - Cue_{er}(e_{i})_{min}}
\vspace{-0.05cm}
\end{equation}

Similarly, given the definitions of \textit{Cues} for KBSs, we capture \textit{the categorization relevance of a KBS}, with the notion of $Focus(K)$, which we define as follows: 

\vspace{-0.2cm}
\begin{equation}
\small
Focus(K) = Cue_{k}^{'}(K) + Cue_{kr}^{'}(K)
\vspace{-0.05cm}
\end{equation}

where $Cue_{k}^{'}(K)$ is a \textit{mean normalization} of $Cue_{k}(K)$, considering all the $Cue_{k}(K)$ values from a given set of KBSs $\left \{ K \right \}$, namely:

\vspace{-0.2cm}
\begin{equation}
\small
Cue_{k}^{'}(K) =\frac{Cue_{k}(K) - Cue_{k}(K_{i})_{average}}{Cue_{k}(K_{j})_{max} - Cue_{k}(K_{k})_{min}}
\vspace{-0.05cm}
\end{equation}

and where $Cue_{kr}^{'}(K)$ is a \textit{min-max normalization} of $Cue_{kr}(K)$ considering all the $Cue_{kr}(K)$ values from a given set of KBSs $\left \{ K \right \}$, namely:

\vspace{-0.2cm}
\begin{equation}
\small
Cue_{kr}^{'}(K) =\frac{Cue_{kr}(K) - Cue_{kr}(K_{i})_{min}}{Cue_{kr}(K_{j})_{max} - Cue_{kr}(K_{i})_{min}}
\vspace{-0.05cm}
\end{equation}

Notice that we used mean normalization for $Cue_{e}(e)$ and $Cue_{k}(K)$ because of the wide range of $Cue_{e}(e)$ and $Cue_{k}(K)$values across the KBSs (e.g., we may have a KBS with  $Cue_{e}(e) = 10$ and a KBS with $Cue_{e}(e) = 300$).



==> sections/draft-images.tex <==
\begin{figure*}[h!]
  \centering
  \begin{subfigure}[b]{0.30\linewidth}
    \includegraphics[width=\linewidth]{images/shared-etypes.png}
    \caption{All properties}
  \end{subfigure}
  \begin{subfigure}[b]{0.30\linewidth}
    \includegraphics[width=\linewidth]{images/dbpedia-shared-properties.png}
    \caption{DBpedia}
  \end{subfigure}
    \begin{subfigure}[b]{0.30\linewidth}
    \includegraphics[width=\linewidth]{images/person.png}
    \caption{Person}
  \end{subfigure}
  \caption{\textit{(a) Shared etypes across resources; (b) Shared properties across etypes; (c) Shared properties across resources.}}
  \label{fig3lotus}
\end{figure*}

\begin{figure}[ht]
  \centering
  \includegraphics[width=\linewidth]{images/00.png}
  \caption{\textit{Contexts properties benchmark: before and after FCA processing}}
  \label{00}
  \vspace{-1em}
\end{figure}

\begin{figure}[ht]
  \centering
  \includegraphics[width=\linewidth]{images/01.png}
  \caption{\textit{Contexts balance benchmark: before and after FCA processing}}
  \label{01}
  \vspace{-1em}
\end{figure}


==> sections/eval2.tex <==
For evaluating Focus(e), we choose xx algorithms as  baseline. Then introduce the reason why we choose these algorithms. Since their is no gold standard of such experiments online, here we collected a manually annotated set of schema and then introduce how we annotated the gold standard data.
After that, we make this evaluation as three steps:
\begin{enumerate}
\item make a comparison between our algorithm and the gold standard, then make a table to show.
\item make a comparison between our algorithm and SoA algorithms, then make a plot.
\item IF there is enough space, discuss how our approach can improve schema tagging tasks
\end{enumerate}





The goal here is \textit{to show how the results discussed above can be correctly predicted by the metrics}; and then, \textit{ to analyze the role of the metrics in the context determination step.} 

Let us start with Sect. \ref{subsec-measuring}.
The results in Table \ref{tab5} map to the ranking of $Cue_{cr}$ in Table \ref{tab8}, where Schema.org has the lowest $Cue_{cr}$, thus showing how this metric, by quantifying the cleanliness of a reference context, can be used to analyse the role of a given reference context. Accordingly, the conclusion that can be drawn is that, \textit{given full coverage (here each context is tested against itself), the higher is the level of contextuality the lower is the level of confusion of contexts in their ability to recognize etypes}.

%CUE-COV-ROLE
%
Let us now consider Sect. \ref{subsec-role}.
From the overall \textit{accuracy} results reported in Fig.~\ref{evalchart} we can observe that the best reference context (Schema.org excluded) in the recognition of the \textit{overall} set of Schema.org etypes is OpenCyc. This is mainly motivated by the fact that, as for the values reported in Table \ref{tab9}, OpenCyc is the reference context \textit{that maximizes the unity with the input context} (see its $Cov_{ci}$ scores). Notice that OpenCyc is not the best context in the \textit{maximization of diversity}, but approaches the best (namely, SUMO, see its $Cue_{cri}$). This fact highlights a stronger impact by $Cov_{ci}$ with respect to $Cue_{cri}$, providing further evidence of what already suggested by the data in
Fig.~\ref{lotus3}, as discussed in Sect. \ref{subsec-role}.
%
The suitability of each context can be also checked at the level of etypes. Looking at each \textit{F1} result reported in Fig.~\ref{evalchart}, we can notice that the best performing etypes are those where the unity with the input context is maximized. However, even when the input is largely covered, a low level of diversity may lead to a decrease in performance, as in the case of Person-OpenCyc vs. Person-DBpedia and Place-OpenCyc vs. Place-SUMO (see Table \ref{tab9}).

The overall conclusion is that \textit{coverage $Cov_{ci}$ is the metric which has the highest impact while the second most important is $Cue_{cri}$ (and $Cue_{eri}$}). This indicates that the algorithm for context determination implements the right strategy and also the possibility to improve its performance via the evaluaton of the best trade-off between the maximization of the unity and the maximization of diversity.

%%%%%%PRICAI

The goals of our case study are: (1) to demonstrate the conceptual power of the Teleo-KR architecture by applying it to a well-known AI task, showing how the latter can be solved through combining classificational and identificational knowledge; and (2) to propose and test a novel idea on the large-scale reuse of existing classificational knowledge for identificational purposes.

The underlying scenario can be described as the \textit{identification of data schemas}: given a set of input \textit{attributes }(or \textit{properties}), find the schema that matches them best. It is a sub-problem of the well-known \textit{schema alignment problem}, used in applications of semantic interoperability, such as data integration or dynamic data matching.

We map this problem onto the Teleo-KR architecture by building a ‘teleological AI agent’. We use this agent to simulate a ‘cognitive cycle’ that starts from perception, identifies the input, builds identificational and classificational knowledge through accumulation and formalisation, respectively, and finally performs a revision of its identificational knowledge to optimise its abilities. We cover the entire cycle through four successive experiments.

==> sections/section2.tex <==
We adapt Rosch's original methodology to the context of knowledge base schema design. In our setting, each available schema (see, for instance, Schema.org or DBpedia) plays the role of a categorization, which is modeled as a set of \textit{entity types} associated with a set of \textit{properties}, whose main function is to \textit{draw sharp lines around the types of entities it contains, so that each member in its domain falls determinately either in or out of each entity type} [Ref.]. The knowledge engineers who devised the schemas play the role of the persons involved in Rosch's experiment. Each knowledge base schema provides a rich set of categorization examples. Each entity type plays the role of a category and all entity type properties play the role of features. The categorization purpose of the schema is then mapped into the notion of \textit{focus}. 
We intuitively model the notion of focus as ``\textit{the state or quality of being relevant in storing and retrieving information}'' and we quantify the degree of this relevance by adapting the Rosch's notion of cue validity as follows:

\begin{itemize}
\item we take each property has to have the same ``cue validity'' (which we assume to be normalized to one). 
\item for each KBS we equally divide the property ``cue validity'' across the entity types the properties are associated to;
\item by checking the wide-spreading of ``cue validity'' we quantify the relevance of schema and entity types in storing and retrieving information.   
\end{itemize}

The ``focus'' can be then calculated in relation to this analysis and, in turn, it can be functionally articulated in:
\begin{itemize}
\item \textit{the entity types focus}, namely, the entity types that are maximally informative categories, namely that maximise the amount of properties and minimize the number of properties. This entity types being, in some extent, related to what expert users consider as ``core entity types'' or most useful etypes for a given domain; 
\item \textit{the schemas focus}, namely the schemas that are straightforwardly identified as maximizing the number of maximally informative (focused) entity types. These schemas being, in some extent, related to what expert users classify as rich, broad and cross-domain knwoledge resources [TBD].
\end{itemize} 

==> sections/section8.tex <==
In this paper we have proposed a formal model and a visual representation of knowledge, when it consists of a set of heterogeneous KBs. This is in turn has allowed us to implement entity type recognition as a multi-label classification problem applied to a set of reference KBs.
The future work will concentrate on a general methodology for re-using, adapting and evolving the large number of existing high-quality KBs.

==> sections/tables.tex <==
\begin{table*}[!htb]
\small
\centering
\setlength{\tabcolsep}{1pt}
\begin{minipage}[t]{.33\linewidth}
\centering
\caption{Focus (entity) scores}
\label{tab:first_table}
\medskip
\begin{tabular}{ccccl}
\toprule
\textit{\textbf{Schema}} & \textit{\textbf{Entity}} & \textbf{$Cue_{e}$} & \textbf{$Cue_{er}$} & \textbf{$Cue_{ec}$} \\ 
\midrule 
A                  & a                  & n                         & n                          & n                           \\
B                  & b                  & n                        & n                           & n                           \\
C                  & c                  & n                           & n                          & n                           \\
D                  & d                  & n                         & n                             & n                             \\ 
\midrule
\end{tabular}
\end{minipage}
\begin{minipage}[t]{.33\linewidth}
\centering
\caption{Shareability (entity) scores}
\label{tab:second_table}
\medskip
\begin{tabular}{ccccl}
\toprule
\textit{\textbf{Schema}} & \textit{\textbf{Entity}} & \textit{\textbf{$Freq_{e}$}} & \textit{\textbf{$Freq_{er}$}} & \textit{\textbf{$Freq_{ec}$}} \\ 
\midrule 
A                  & a                  & n                          & n                          & n                           \\
B                  & b                  & n                         & n                          & n                           \\
C                  & c                  & n                            & n                           & n                          \\
D                  & d                  & n                         & n                             & n                             \\ 
\midrule
\end{tabular}
\end{minipage}\hfill
\begin{minipage}[t]{.33\linewidth}
\centering
\caption{Overall (entity) scores}
\label{tab:third_table}
\medskip
\begin{tabular}{ccccl}
\toprule
\textit{\textbf{Schema}} & \textit{\textbf{Entity}} & \textit{\textbf{$Scr_{search}(e)$}} & \textit{\textbf{$Scr_{share}(e)$}} & \textit{\textbf{$Scr_{all}(e)$}} \\ 
\midrule 
A                  & a                  & n                          & n                           & n                           \\
B                  & c                  & n                        & n                           & n                           \\
C                  & f                  & n                            & n                          & n                           \\
D                  & h                  & n                         & n                             & n                             \\ 
\midrule
\end{tabular}   
\end{minipage} 
\end{table*}

\begin{table*}
\caption{Focus, shareability and overall (context) scores}
\label{tab:fourth_table}
\centering
\begin{tabular}{ccccllllll}
\toprule
\textit{\textbf{Schema}} & \textit{\textbf{$Cue_{c}$}} & \textit{\textbf{$Cue_{cr}$}} & \textit{\textbf{$Cue_{cc}$}} & $Freq_{c}$ & $Freq_{cr}$ & $Freq_{cc}$ & \textit{\textbf{$Scr_{search}(C)$}} & $Scr_{share}(C)$ & $Scr_{all}(C)$ \\ \midrule
A                  & n                      & n                       & n                       & n     & n      & n      & n                        & n       & n            \\
B                  & n                      & n                       & n                       & n     & n      & n      & n                        & n       & n            \\
C                  & n                      & n                       & n                       & n     & n      & n      & n                        & n       & n            \\
D                  & n                      & n                       & n                       & n     & n      & n      & n                        & n       & n            \\
\midrule
\end{tabular}
\end{table*}




%tab1
\begin{table}[]
\caption{\textit{text}}
  \label{tab1}
\centering
\small
\begin{tabular}{ccccc}
\hline
\textbf{schema}    & \textbf{class}                & \textbf{$Cue_{e}(e)$}   & \textbf{$Cue_{er}(e)$} & \textbf{$Score(e)$} \\ \hline
\textit{dbpedia:}  & \textit{person}               & \textbf{169,02} & \textbf{0,69}  & \textbf{1,42}  \\
\textit{opencyc:}  & \textit{firstordercollection} & \textbf{230,59} & \textbf{0,30}  & \textbf{1,30}  \\
\textit{freebase:} & \textit{statisticalregion}    & \textbf{161,53} & \textbf{0,48}  & \textbf{1,17}  \\
\textit{opencyc:}  & \textit{class}                & \textbf{194,95} & \textbf{0,31}  & \textbf{1,15}  \\
\textit{dicom:}    & \textit{ieimage}              & \textbf{158,90} & \textbf{0,44}  & \textbf{1,13}  \\
\textit{dbpedia:}  & \textit{place}                & \textbf{116,97} & \textbf{0,63}  & \textbf{1,13}  \\
\textit{SUMO:}     & \textit{geopoliticalarea}     & \textbf{85,23}  & \textbf{0,75}  & \textbf{1,12}  \\
\textit{gndo:}     & \textit{work}                 & \textbf{59,56}  & \textbf{0,85}  & \textbf{1,10}  \\
\textit{opencyc:}  & \textit{agentgeneric}         & \textbf{170,09} & \textbf{0,37}  & \textbf{1,10}  \\
\textit{opencyc:}  & \textit{intelligentagent}     & \textbf{168,80} & \textbf{0,37}  & \textbf{1,10}  \\
\textit{opencyc:}  & \textit{partiallytangible}    & \textbf{165,90} & \textbf{0,38}  & \textbf{1,09}  \\ \hline
\end{tabular}
\end{table}

\begin{table}[]
\caption{\textit{text}}
  \label{tab2}
\centering
\small
\begin{tabular}{ccccc}
\hline
\textbf{schema}    & \textbf{class}  & \textbf{$Cue_{e}(e)$}   & \textbf{$Cue_{er}(e)$} & \textbf{$Score(e)$} \\ \hline
\textit{dbpedia:}  & \textit{person} & \textbf{169,02} & \textbf{0,69}  & \textbf{1,42}  \\
\textit{akt:}      & \textit{person} & \textbf{8,00}   & \textbf{1,00}  & \textbf{1,03}  \\
\textit{opencyc:}  & \textit{person} & \textbf{122,14} & \textbf{0,43}  & \textbf{0,95}  \\
\textit{vivo:}     & \textit{person} & \textbf{10,60}  & \textbf{0,88}  & \textbf{0,92}  \\
\textit{swpo:}     & \textit{person} & \textbf{3,50}   & \textbf{0,88}  & \textbf{0,88}  \\
\textit{cwmo:}     & \textit{person} & \textbf{5,83}   & \textbf{0,83}  & \textbf{0,85}  \\
\textit{earth:}    & \textit{person} & \textbf{2,50}   & \textbf{0,83}  & \textbf{0,84}  \\
\textit{nlon:}     & \textit{person} & \textbf{2,50}   & \textbf{0,83}  & \textbf{0,84}  \\
\textit{schema:}   & \textit{person} & \textbf{34,86}  & \textbf{0,52}  & \textbf{0,67}  \\
\textit{pext:}     & \textit{person} & \textbf{8,13}   & \textbf{0,58}  & \textbf{0,61}  \\
\textit{freebase:} & \textit{person} & \textbf{37,07}  & \textbf{0,27}  & \textbf{0,43}  \\ \hline
\end{tabular}
\end{table}
